Formal Verification, Engineering and Business Value

How to apply automated verification technology such as model checking and static program analysis to millions of lines of embedded C/C++ code? How to package this technology in a way that it can be used by software developers and engineers, who might have no background in formal verification? And how to convince business managers to actually pay for such a software? This work addresses a number of those questions. Based on our own experience on developing and distributing the Goanna source code analyzer for detecting software bugs and security vulnerabilities in C/C++ code, we explain the underlying technology of model checking, static analysis and SMT solving, steps involved in creating industrial-proof tools.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{C.\ Artho and P.C.\ \"Olveczky (Eds.): FTSCS 2012\\
EPTCS 105, 2012, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.105.1}{10.4204/EPTCS.105.1}}
\pdfoutput=1

